Moment-Based 3D Gaussian Splatting: Resolving Volumetric Occlusion with Order-Independent Transmittance

The recent success of 3D Gaussian Splatting (3DGS) has reshaped novel view synthesis by enabling fast optimization and real-time rendering of high-quality radiance fields. However, it relies on simplified, order-dependent alpha blending and coarse approximations of the density integral within the rasterizer, thereby limiting its ability to render complex, overlapping semi-transparent objects. In this paper, we extend rasterization-based rendering of 3D Gaussian representations with a novel method for high-fidelity transmittance computation, entirely avoiding the need for ray tracing or per-pixel sample sorting. Building on prior work in moment-based order-independent transparency, our key idea is to characterize the density distribution along each camera ray with a compact and continuous representation based on statistical moments. To this end, we analytically derive and compute a set of per-pixel moments from all contributing 3D Gaussians. From these moments, a continuous transmittance function is reconstructed for each ray, which is then independently sampled within each Gaussian. As a result, our method bridges the gap between rasterization and physical accuracy by modeling light attenuation in complex translucent media, significantly improving overall reconstruction and rendering quality.

==> chapters/03_method/theory.tex <==
\section{Theoretical Background}
Let $\tau : \mathbb{R} \to \mathbb{R}$ be a monotonic increasing and right continuous function. Then, there exists a unique measure $\mu_\tau$ on the measurable space $(\mathbb{R}, \mathcal{B}(\mathbb{R}))$, called the \textit{Lebesgue-Stieltjes measure} which satisfies the property 
\begin{equation*}
    \mu_\tau((a,b]) = \tau(b) - \tau(a).
\end{equation*}
Furthermore, if $\tau$ is absolutely continuous, then its associated measure $\mu_\tau$ is absolutely continuous with respect to the Lebesgue measure $\lambda$ (denoted $\mu_\tau  \ll \lambda$). The Radon–Nikodym theorem then guarantees the existence of a measurable function $\sigma: \mathbb{R} \to [0, \infty)$, such that for any measurable set $B \in \mathcal{B}(\mathbb{R})$,
\begin{equation*}
    \mu_\tau(B) = \int_{B} \sigma \, \dd \lambda.
\end{equation*}
The function $\sigma$ is called the (Radon-Nikodym) density of $\mu_\tau$ with respect to $\lambda$ (denoted $\sigma = \frac{d\mu_\tau}{d\lambda}$) and is given by the derivative of $\tau$, i.e.,  $\sigma(x) = \tau'(x)$ for almost every $x \in \mathbb{R}$.

For a given positive measure $\mu$ on $\mathbb{R}$, its $k$-th raw moment is defined by the integral
\begin{equation*}
    m_k = \int_{-\infty}^{\infty} x^k \, \dd \mu(x),
\end{equation*}
provided the integral converges absolutely. In the special case where $\mu$ is absolutely continuous with respect to the Lebesgue measure,  the moment can be written as in terms of its density $\sigma(x)$.

The "moment problem" addresses the inverse question: for a given sequence $(m_k)_{k \geq 0}$  of real numbers is asks: 
\begin{enumerate}
    \item Existence: Does there exists a positive measure on $\mu$ on $\mathbb{R}$ such that its moments are the sequence $(m_k)_{k \geq 0}$?
    \item Uniqueness: If such a measure exists, it is uniquely determined by this sequence of moments?
    \item Characterization: If the measure is not unique, how can one describe the set of all measures with these moments?
\end{enumerate}
In general, a finite number of moments does not characterize a unique measure. The full infinite sequence is required to even have a change at uniqueness. Fortunately, a lower and upper bounds on the set of measures characterized by the finite moments
\begin{equation*}
    \begin{split}
    \mu_L(x) &= \inf \left\{ \mu(x) \mid m_k = \int_{-\infty}^{\infty} x^k \, \dd \mu(x)\right\} \\
    \mu_U(x) &= \sup \left\{ \mu(x) \mid m_k = \int_{-\infty}^{\infty} x^k \, \dd \mu(x)\right\},   
    \end{split}
\end{equation*}
can be computed with only mild assumption about the moment \TODO{Citation needed}.

These bounds have been extensively studied in real-time graphics methods to approximate complex occlusions in shadow mapping \cite{peters2015moment, peters2016beyond, peters2017improved, peters2017non}, and more relevant to this work, have been applied to order-independent transparency \cite{munstermann2018moment}. The latter application models occlusion along a view ray via an absorbance function $A(z)=-\ln T(z)$, with $T(z)$ being the transmittance at depth $z$. For $N$ discrete transparent surfaces at depths $z_l$ with opacities $\alpha_l$, the absorbance function is a monotonic, right-continuous step function \cite{munstermann2018moment}:
\begin{equation*}
A(z) = \sum_{l=0, z_l < z}^{N-1} -\ln(1-\alpha_l).
\end{equation*}
This function $A(z)$ is an instance of $\tau(z)$ from the preceding theory. The associated Lebesgue-Stieltjes measure $\mu_A$ is a sum of weighted Dirac delta functions, where each surface corresponds to a point mass:
\begin{equation*}
\mu_A = \sum_{l=0}^{N-1} w_l \delta_{z_l}, \quad \text{with weights } w_l = -\ln(1-\alpha_l).
\end{equation*}
Rather than storing the full measure, its first $2n+1$ moments, $m_k=\int z^k \dd \mu_A(z)$, are computed and stored per pixel. To reconstruct the bounds on the absorbance at a query depth $\eta$, a unique canonical representation of the moments is constructed. This representation is itself a discrete measure, $\tau_\eta = \sum_{i=0}^n w_i' \delta_{x_i}$, with $n+1$ points of support that has the same moments as $\mu_A$ and is constrained such that one of its support points is the query depth itself, i.e., $x_0=\eta$ \cite{worchel2025moment}.

The problem is thus reduced to finding the unknown locations $\{x_i\}_{i=1}^n$ and weights $\{w_i'\}_{i=0}^n$. The locations are found as the roots of the degree-n kernel polynomial $K(x)=x^T H^{-1} \eta$, where $H$ is the Hankel matrix of the moments ($H_{ij}=m_{i+j}$). Once the locations $\{x_i\}$ are known, the weights are found by solving the linear Vandermonde system given by the moment equations $m_k=\sum_{i=0}^n w_i' x_i^k$. Finally, the bounds are computed from this discrete measure:
\begin{equation*}
L(\eta) = \sum_{x_i < \eta} w_i' \quad \text{and} \quad U(\eta) = \sum_{x_i \le \eta} w_i'.
\end{equation*}
Recent work has proven that the moment-bounds, even though piecewise constant, are differentiable \cite{worchel2025moment}.

